Finishing Flows Quickly with Preemptive Scheduling

Today's data centers face extreme challenges in providing low latency. However, fair sharing, a principle commonly adopted in current congestion control protocols, is far from optimal for satisfying latency requirements. We propose Preemptive Distributed Quick (PDQ) flow scheduling, a protocol designed to complete flows quickly and meet flow deadlines. PDQ enables flow preemption to approximate a range of scheduling disciplines. For example, PDQ can emulate a shortest job first algorithm to give priority to the short flows by pausing the contending flows. PDQ borrows ideas from centralized scheduling disciplines and implements them in a fully distributed manner, making it scalable to today's data centers. Further, we develop a multipath version of PDQ to exploit path diversity. Through extensive packet-level and flow-level simulation, we demonstrate that PDQ significantly outperforms TCP, RCP and D3 in data center environments. We further show that PDQ is stable, resilient to packet loss, and preserves nearly all its performance gains even given inaccurate flow information.

==> NOTES <==
Like most new transport protocols, our design requires changes
to certain parts of the network.
However, \name can be 

to be deployed, name requires changes to switches within the ntwork.
however, \name can be deployed

Implementing \name within a switch

In previous sections, we described  name.
name has a few requiremnets from switches
- periodically sample flow rates
- need to modify (flow rate) fields in packets
- maintain flow list data structure
- perofrm cmputation on the flow list to derive new flow rates
to support this funcitonality, we need to make modifications to the switch.

Commercial switches can be thought of as specialized computers.  Like
traditional computers, they often run {\em software}: an operating system and
collection of protocol daemons that run atop a microprocessor.  The software of
a switch is used to implement routing protocol logic, configuration and vty
functionality, etc.  To support high-speed packet forwarding, switches often
also have customized {\em hardware}, often in the form of a customized ASIC.
This hardware support queuing, destination port lookup, filtering, matching,
and other operations that must be supported at high speed.  The switch's
software can control the hardware's operations through an interface, for
example, by writing into memory banks that are read directly by the switch's
hardware.

In previous sections (Sections~\ref{xx-xx}, we described the switch-level
operational requirements of \name.  \name requires the ability to periodically
sample flow rates, to maintain a flow list data structure, to perform a
computation on the flow list to derive new flow rates, and to modify fields in
packet headers.  A vendor can implement \name in a switch by making
modifications to the switch's hardware and software.  For example, operations
that must be done per-packet at high speeds (flow rate sampling and modifying
header fields)  can be implemented by modfiying the switch's ASIC.  More
complex operations that do not need to be done in real time can be implemented
in software (computing the current set of flow rates for header fields, and
maintaining the flow list).  \mattc{double check with CY: this computation
isn't done per packet, right? the computation doesn't need to be done in real
time right?} \name's hardware operations are limited to flow rate sampling and
modifying header fields, which can be done with straightforward modifications
to device hardware.

To improve deployability, we would like to avoid requiring vendors to make
hardware-level changes to their existing switches.  To support this, we
describe how \name can be deployed through software-only modifications if the
vendor's equipment already supports OpenFlow.  OpenFlow is a technology that
exposes a set of APIs to allow fine-grained control over network forwarding
behavior.  To implement OpenFlow within a network device, the vendor extends
the hardware to provide customizable control on packet forwarding behavior, and
an interface to allow switch software to control this functionality.  The
vendor also implements the OpenFlow protocol, to enable a centralized
controller to control the switch's functionality.  \name makes use of the
former, but not the latter.  In particular, \name can be implemented as a set
of extensions to the software running at a switch, that exploits the local
OpenFlow hardware interfaces developed by the vendor.  \name's hardware
operations (flow rate sampling and modifying header fields) can then be done by
directly manipulating OpenFlow rules (using matching and counters for flow rate
sampling, and actions for modifying header fields). As before, the remainder of
\name's functionality can be implemented to the software running at the switch.

However, to improve deployability, we would like to avoid requiring
hardware-level changes to switches. 



one way to do this would be to modify switch hardware and software.


for example, the equipment vendor 

as an alternative, equipment vendors that already support openflow can instrument
our techniques with only a software patch to their existing devices.



openflow is a technology that exposes a set of APIs to allow fine-grained
control over netowk forwarding behavior.
To implement OpenFlow within a network device, the vendor constructs a set of
modifications to the device's hardware to correspond to the OpenFlow
specification. The vendor the constructs a hardware API to software. Within
software, the vendor 
aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa

{\em Datacenters} are now used as the underlying infrastructure of many modern
commercial operations, including web services, cloud computing,  and some of
the world's largest databases and storage services.  Because of this, modern
datacenter networks face some of the most challenging workloads of any network
in existance. In particular, data centers face two key unique challenges:

* Extremely large workloads: 

* Strong applicaiton demands


{\em Datacenters} are now used as the underlying infrastructure of many modern
commercial operations, including web services, cloud computing,  and some of
the world's largest databases and storage services.  Because of this, modern
datacenter networks face some of the most large-scale workloads of any network
in existence.  Unfortunately, datacenters also often host applications with
very demanding real-time requirements, including financial services,
multimedia, communications services, and web search.  Meeting these
requirements in this challenging environment is a very challenging problem.

To meet this challenge, we need some way to effectively divide up the bandwidth
of the network across the different jobs that the data center network is
running. To cope with modern datacenters' large-scale workloads, we would like
to maximize the {\em throughput}, or number of jobs that can be completed per
unit time. To cope with datacenters' application demands, we would like to
ensure that the number of jobs that meet application deadlines is as high as
possible.

How can we solve this problem? One approach would be to apply existing
transport mechanisms, such as TCP, RCP, ICTCP, and DCTCP. However, these
mechanisms were designed with a different goal in mind. These approaches work
by targeting {\em fair sharing} of network capacity---link bandwidth is equally
divided across flows.  While fair sharing is a useful approach for environments
where a resource should be divided evenly over participants, for example
environments with uncooperative hosts, fair sharing is known to be far from
optimal in terms of minimzing flow completion time, and the number of flows
that meet their deadlines.

This paper takes a different approach. In particular, we propose \sys, a scheme
that  leverages ideas developed in the context of real-time operating systems
to perform {\em dynamic scheduling} of flows in a data center.  The main
observation is that the problem of optimally scheduling a set of tasks for a
shared resource, with the goal of maximizing throughput, is not a new problem.
In the context of real-time operating systems, a class of {\em dynamic
scheduling algorithms} have been developed that are known to be optimal for
this problem.  For example, the Earliest Deadline First (EDF) dynamic
scheduling policy, which stores a queue of tasks sorted by deadlines and
repeatedly selects the task with nearest deadline for scheduling, is known to
be optimal: if there is a set of jobs with deadlines, and there exists a
schedule that enables all jobs to be completed before their deadlines, EDF will
complete those jobs by their deadlines.  For tasks without deadlines, Shortest
Job First (SJF) is known to maximize process throughput, as well as minimizing
the amount of time each process needs to wait before its execution is complete.
In addition to providing strong properties, these algorithms also significantly
outperform more simple scheduling disciplines, as shown by our results, where
we compare against schemes based on FCFS (e.g., D3~\cite{xx}) and fair sharing.

However, dynamic scheduling policies such as EDF and SJF were developed in the
context of centralized environmnets. Applying these ideas to a distributed
datacenter environment introduces several new challenges.  First, centralized
dynamic scheduling relies on the ability to {\em preempt} an existing task, to
ensure a newly arriving task with a smaller deadline is able to be completed
before a currently-scheduled task. To support this task in distributed
environments, \sys provides the ability to perform distributed preemption of
existing flow traffic, in a manner that enables fast switchover and is
guaranteed not to lead to deadlock.  Second, centralized dynamic scheduling
assumes that the global state of the system is known to the scheduler, and that
scheduling is done at a single point.  To perform dynamic scheduling in
decentralized environments, \sys provides a distributed algorithm to allow a
set of switches to collaboratively gather information about flow workloads, and
converge to a stable agreement on allocation decisions.

Through an extensive simulation study leveraging real datacenter workloads, we
find that \sys provides strong benefits over existing datacenter transport
mechanisms.  For deadline-constrained flows, \sys outperforms \bntl by
supporting $3$ times more concurrent senders while satisfying their flow
deadlines.  When flows have no deadlines, we show \sys can reduce flow
completion times by $\sim$$30\%$ as compared with TCP and RCP \mattc{and D3?
Can I say D3 here?}.















istribute and schedule flow traffic in a manner that 


 such as FCFS and fair sharing on a wide
variety of practical workloads. 

which repeatedly schedules the task with nearest deadline





However, the problem of scheduling a set of tasks to maximize metrics such as 
throughput and flow 
In the context of 



This paper takes a different approach. 

In particular, we argue that
the problem of scheduling a set of tasks to maximize metrics such as through









How can we efficiently utilize a data center's network? One approach
would be to apply existing transport mechanisms, such as TCP, RCP, ICTCP,
and DCTCP. These approaches work by targeting {\em fair sharing} of network
capacity---link bandwidth is equally divided across flows.
However, the goal of fair sharing does not match with the 
To build data centers that can cope with large scale workloads, we need
to maximize {\em throughput}



However, fair sharing faces several problems.
First, to cope with large-scale workloads, datacenters need to maximize throughput,
by completing as many jobs as possible within a fixed period of time.
Second





However, fair sharing faces several problems
- first of all flows often need to complete by certain times. so need to take that into account
- also it's important to 


However, fair sharing is known to be far from optimal in terms of 
metrics that matter to data center applications, such as flow completion
time, and the number of flows that miss their deadline.





How can we solve this problem?
One approach would be to apply existing transport mechanisms to this problem
TCP/RCP/etc. 
however, these approaches were designed to ensure fair sharing of the
network's capacity. 
this was a reasonable approach in wide-area networks, where hosts are uncooperative and fair sharing across them seemed like a reasonable goa.
however in datacenters we have a new opportunity, as we can schedule things precisely



To cope with this problem, modern datacenters make use of transport mechanisms

The problem of efficiently sharing a network's 

One approach to this problem would be to apply 





designing transport mechanisms for
data center traffic an extremely challenging problem.





Providing efficient use of network resources while simultaneously
meeting the requirements of applications which often have real-time demands
on service time makes the problem of efficiently scheduling traffic


on the ability to complete traffic
makes the problem of efficiently scheduling traffic within a datacenter
to be an 




Coupled with demanding application
requirements, this means that the ability to efficieintly transport
data within a datacenter is an increasingly critical challenge.



Datacenters are used as the backbone of many modern commercial
operations, from web services to cloud computing to XX.
Their increasing pervasiveness means modern datacenters must cope with 
a 

datacenters are very important, 
network is a bottleneck -- very network intense, massive workloads need to be transferred around
in order to make them perform efficiently, we need to make different hosts efficiently share the network

traditional approach to this was to do fair sharing across flows. use of tcp/etc in the wide area. this approach as useful in the wide area because 
hosts were competing. in the data center, there's a new opportunity because
you know global state about the workload

to leverage this opportunity, we argue that we should do flow scheduling





Our approach has two benefits
- flexibliity to use arbitrary scheduling disciplines, giving operator the ability to select disciplines that match their workload
- use of more advnaced scheduling disciplines


FCFS is only optimal when the sequence of deadlines matches the arrival times of flows.
We show in later sections this greatly decreases D3's performance in practice.





==========

req, fair share,

edf is packet based -
leads to congestion collapse -
distributed rate control scheme is not trivial
req priority queue at routers - bc do pausing and flow-level

you do edf
- distributed scheme
- pausing
- flow-level

we do edf for deadline constrainted flows
and sjf for deadline unconstirained flows

two kids of scheduling
fixed priority - flow's priority is fixed over time
dynamic - whenever there's a new flow coming in or terminates every flow's         priority coudl change

ability to schedule flows based on a specific order

you can handle arbitrary orderings

aaaaaaaaa

a scheme that upports arbitrary flow schedulig
we apply this to preemption-based scheduling
a

what changes do we need at a host



==> intro-old.tex <==
\section{Introduction (Chi-Yao)}
\label{sec:introduction}

Datacenters are now used as the underlying infrastructure of many modern
commercial operations, including web search, databases, financial and storage services. 
These applications often require the shortest possible response time, 
as users want their results as fast as possible.
Some soft real-time applications even have latency targets to meet, requiring 
network flows to complete before certain deadlines~\cite{dctcp}.
Unfortunately, transport protocols like TCP are neither minimizing
flow completion time nor optimizing for deadlines, resulting in the fact that a significant fraction of 
flow deadlines are missed in today's data centers~\cite{bntl}.

Until now, \emph{fair sharing} -- link bandwidth is equally divided among flows -- 
is a long-established objective adopted by current congestion control protocols in data centers 
such as TCP, RCP\cite{rcp}, ICTCP~\cite{ictcp} and DCTCP~\cite{dctcp}. 
In particular, these protocols will gradually converge on the fair-share allocation among flows.
However, fair sharing is known to be far from optimal in terms of minimizing flow completion time~\cite{PShaslargeFCT} 
and the number of deadline-missing flows~\cite{EDFbetterthanPS}.
%\cut{XCP\cite{xcp}}

Arguably, \emph{flow scheduling}\footnote{We refer flow scheduling to sequencing flow transmission order in \emph{time}. 
This differs from the flow scheduler in Hedera~\cite{hedera} which assigns flows to \emph{paths}.} 
is the most persuasive solution to this problem:
Rather than allowing all flows to transmit at the same time, one 
could leverage scheduling theory to resequence flow transmission order, 
achieving optimum in many scenarios. 
Consider a single bottleneck link: Transmitting flows one after one in increasing order of flow 
size (Shortest Job First; SJF) is optimal to minimize average flow completion time~\cite{srptoptimality};
if flows are annotated with deadlines, transmitting flows in increasing order 
of deadline (Earliest Deadline First; EDF) is optimal to find a deadline-satisfying solution if any exists~\cite{edfoptimality}.
As we will show in later section, these scheduling disciplines have clear performance advantages over 
existing congestion control protocols even for more complex scenarios (e.g., multi-rooted tree topology, dynamic traffic loads).

%In this paper we start with the assumptions that \textbf{\small(i)} minimizing flow completion time (for flows without deadline) and 
%satisfying flow deadline requirements (for deadline-constrained flows) at the same time 
%plays an important, perhaps even necessary, role in data center networks, and \textbf{\small(ii)} the use of fair sharing in existing transport protocols is 
%a substantial hindrance to achieve this goal.
%We are not claiming that they are true, but rather are only 
%looking at the implications if indeed they are true by using these two
%assumptions as our starting points. If one starts with these assumptions, 
%then designing a new congestion control protocol to achieve this goal becomes a very important issue.

%To address this problem, 
%this paper develops a novel protocol for congestion control that
%outperforms state-of-the-art transport protocols in data center networks.

%Since it seems that \emph{fair} sharing hinders flow completion time, we propose the opposite: 
%giving high priority to certain flows chosen by a scheduling discipline. 
Therefore, we propose the opposite to \emph{fair} sharing: Giving priority to certain flows chosen by a scheduling discipline.
This scheduling-based congestion control protocol, called Preemptive Distributed Quick scheduling (\textbf{\sys{}}), is 
efficient, error-resilient, and scalable to current data center size. 
It borrows the ideas from centralized scheduling disciplines and 
implements it in a fully distributed manner. 
With explicit rate control, \sys can approximate a range of scheduling disciplines by 
suitably manipulating the flow transmission time. To achieve this, 
\sys exhibits a unique feature that differentiates it from other congestion control protocols.
We refer this feature as \emph{preemption}:
A scheduling discipline first defines how critical a network flow is, and \sys is capable to give 
priority to the most critical flows while pausing the other contending flows at 
the same time regardless of flow arrival time. This distinctive feature substantially influences the performance: 
In a deadline-constrained case, an urgent flow can ``preempt'' other flows to meet its deadline constraint. 
As we will later show, preemption is very useful to minimize flow completion time even when flows have no deadlines.

To schedule flow transmission time, \sys switches collaboratively converge to a stable agreement and 
inform the senders about the time to start their transmission.
By putting flow information in the packets,
switches need no additional standalone control message, maintain no per-flow state, 
use only FIFO tail-drop queue and require no synchronized clock.

Like D$^3$, a recent deadline-aware protocol proposed by Wilson et al.~\cite{bntl}, 
\sys requires flow information like flow size and deadline at flow initiation time. 
Unlike D$^3$, which is in spirit a first-come first-serve algorithm, \sys gives network resources to the most critical 
flow, approximating the optimal schedule and outperforming D$^3$.
We discuss in~\S\ref{sec:discussion} why the flow size information is available in data center networks, and 
even if this information is inaccurate, we show that \sys performance will 
degrade slowly and gracefully as inaccuracy increases in~\S\ref{sec:badcases}.

%Through both packet-level and flow-level simulation, we observe clear benefits at many network sizes, ranging from a single 
%bottleneck topology to a Fat-tree~\cite{fattree} topology with thousands of servers. 
Inspired by recent proposal on multipath TCP~\cite{mptcp,mptcp-nsdi}, we also develop a multipath version of \sys in \S\ref{sec:multipath}.
By exploiting path diversity, the multipath \sys further improves reliability and flow completion time from the single-path \sys.

%We looked at BCube~\cite{bcube}, multi-homed data center topologies, to take advantage of parallel paths between hosts.
%In random permutation traffic, we show that $4$-subflow \sys can support twice the number of concurrent flows with tight deadlines than single-path \sys.

In summary, our key contributions include:
\begin{itemize}
%\item A scheme to support arbitrary scheduling
%\item We apply this to minimize flow completiont time or the number of deadline-missing flows.
\item We design and implement \sys, a fully distributed protocol that optimizing flow completion time in data centers based on scheduling disciplines.
\item We demonstrate \sys provides significant advantages over state-of-the-art congestion control protocols.
We show \sys can save $\sim$$30\%$ average flow completion time compared with TCP, RCP and \bntl.
For deadline-constrained flows, \sys outperforms \bntl in supporting $3$ times
more concurrent senders while satisfying their flow deadlines. 
\item We show that \sys is stable, resilient to packet loss and inaccurate flow information, while retaining its performance gains at today's data center scale.
\item We develop and evaluate a multipath version of \sys. By exploiting path diversity, we demonstrate that multipath \sys further improves its  
performance and reliability from the single-path \sys.
\end{itemize}

\textbf{Outline:} Next, we discuss an example of benefits~(\S\ref{sec:benefits}), followed by a description of design goals~(\S\ref{sec:challenges}).
%challenges to apply scheduling disciplines to data center flows 
We then present \sys protocol~(\S\ref{sec:algorithm}) and its 
basic properties~(\S\ref{sec:properties}). We demonstrate how \sys works~(\S\ref{sec:dynamic}), followed by a thorough 
performance evaluation (\S\ref{sec:evaluation}), and an analysis of failure resilience (\S\ref{sec:badcases}) using both 
packet-level and flow-level simulation. We then extend to Multipath \sys and demonstrate its effectiveness (\S\ref{sec:multipath}).
Finally, we discuss the protocol limitations~(\S\ref{sec:discussion}), related work (\S\ref{sec:relatedwork}) and conclude~(\S\ref{sec:conclusion}).
%present \sys implementation~(\S\ref{sec:implementation}), 
%Finally, we discuss 





==> introcy.tex <==
\section{Introduction OLD}
\label{sec:introduction2}

Almost any network flow in data centers is preferable to finish early, as users always want to get their results in the shortest time. 
Some flows even have specified deadline to meet because of the soft real-time nature of data center applications such as web search, 
retail, advertising, and recommendation systems. 
Consequently, a deadline-constrained flow is useful if and only if it completes before the deadline~\cite{dctcp}.
Unfortunately, transport protocols like TCP are neither minimizing
flow completion time nor optimizing for deadlines, resulting in the fact that a significant fraction of 
flow deadlines are missed in today's data centers~\cite{bntl}.

Until now, \emph{fair sharing} -- link bandwidth is equally divided among flows -- 
is a long-established objective adopted by current congestion control protocols in data centers 
such as TCP, RCP\cite{rcp}, ICTCP~\cite{ictcp} and DCTCP~\cite{dctcp}. 
In particular, these protocols will gradually converge on the fair-share allocation among flows.
However, fair sharing is known to be far from optimal in terms of minimizing flow completion time~\cite{PShaslargeFCT} 
and the number of deadline-missing flows~\cite{EDFbetterthanPS}.
%\cut{XCP\cite{xcp}}

Arguably, \emph{flow scheduling}\footnote{We refer flow scheduling to sequencing flow transmission order in \emph{time}. 
This differs from the flow scheduler in Hedera~\cite{hedera} which assigns flows to \emph{paths}.} 
is the most persuasive solution to this problem:
Rather than allowing all flows to transmit at the same time, one 
could leverage scheduling theory to resequence flow transmission order, 
achieving optimum in many scenarios. 
Consider a single bottleneck link: Transmitting flows one after one in increasing order of flow 
size (Shortest Job First; SJF) is optimal to minimize average flow completion time~\cite{srptoptimality};
if flows are annotated with deadlines, transmitting flows in increasing order 
of deadline (Earliest Deadline First; EDF) is optimal to find a deadline-satisfying solution if any exists~\cite{edfoptimality}.
As we will show in later section, these scheduling disciplines have clear performance advantages over 
existing congestion control protocols even for more complex scenarios (e.g., multi-rooted tree topology, dynamic traffic loads).

%In this paper we start with the assumptions that \textbf{\small(i)} minimizing flow completion time (for flows without deadline) and 
%satisfying flow deadline requirements (for deadline-constrained flows) at the same time 
%plays an important, perhaps even necessary, role in data center networks, and \textbf{\small(ii)} the use of fair sharing in existing transport protocols is 
%a substantial hindrance to achieve this goal.
%We are not claiming that they are true, but rather are only 
%looking at the implications if indeed they are true by using these two
%assumptions as our starting points. If one starts with these assumptions, 
%then designing a new congestion control protocol to achieve this goal becomes a very important issue.

%To address this problem, 
%this paper develops a novel protocol for congestion control that
%outperforms state-of-the-art transport protocols in data center networks.

Since it seems that \emph{fair} sharing hinders flow completion time, we propose the opposite: 
giving high priority to certain flows chosen by a scheduling discipline. 
This Scheduling-based transmission Control Protocol (\textbf{\sys{}}) is 
%, outperforms state-of-the-art congestion control protocols in data center networks, 
efficient, error-resilient, and scalable to current data center size. 
It borrows the ideas from centralized scheduling disciplines and 
implements it in a fully distributed manner. 
With explicit rate control, \sys can approximate a range of scheduling disciplines by 
suitably manipulating the flow transmission time. To achieve this, 
\sys exhibits a unique feature that differentiates it from other congestion control protocols.
We refer this feature as \emph{preemption}:
A scheduling discipline first defines how critical a network flow is, and \sys is capable to give 
priority to the most critical flows while pausing the other contending flows at 
the same time regardless of flow arrival time. This distinctive feature substantially influences the performance: 
In a deadline-constrained case, an urgent flow can ``preempt'' other flows to meet its deadline constraint. 
As we will later show, preemption is very useful to minimize flow completion time even when flows have no deadlines.

To schedule flow transmission time, \sys switches collaboratively converge to a stable agreement and 
inform the senders about the time to start their transmission.
By putting flow information in the packets,
switches need no additional standalone control message, maintain no per-flow state, use only FIFO tail-drop queue and require no synchronized clock.

Like D$^3$, a recent deadline-agnostic protocol proposed by Wilson et al.~\cite{bntl}, 
\sys requires flow information like flow size and deadline at flow initiation time. 
Unlike D$^3$, which is in spirit a first-come first-serve algorithm, \sys gives network resources to the most critical 
flow, approximating the optimal schedule and outperforming D$^3$.
We discuss in~\S\ref{sec:discussion} why the flow size information is available in data center networks, and 
even if this information is inaccurate, we show that \sys performance will 
degrade slowly and gracefully as inaccuracy increases in~\S\ref{sec:badcases}.

Through both packet-level and flow-level simulation, we observe clear benefits at many network sizes, ranging from a single 
bottleneck topology to a Fat-tree~\cite{fattree} topology with thousands of servers. 
Inspired by recent proposal on multipath TCP~\cite{mptcp,mptcp-nsdi}, we also develop a multipath version of \sys in \S\ref{sec:multipath}.
By exploiting path diversity, the multipath \sys further improves reliability and flow completion time from the single-path \sys.

%We looked at BCube~\cite{bcube}, multi-homed data center topologies, to take advantage of parallel paths between hosts.
%In random permutation traffic, we show that $4$-subflow \sys can support twice the number of concurrent flows with tight deadlines than single-path \sys.

In summary, our key contributions include:
\begin{itemize}
\item We design and implement \sys, a fully distributed protocol that optimizing flow completion time in data centers based on scheduling disciplines.
\item We have examined many traffic patterns and topologies, and in 
all of them \sys provides significant advantages over state-of-the-art congestion control protocols.
For deadline-constrained flows, \sys outperforms \bntl in supporting $3$ times
more concurrent senders while satisfying their flow deadlines. 
When flows have no deadlines, we show \sys can save $\sim$$30\%$ average flow
completion time compared with TCP and RCP.
\item We show that \sys has no deadlock and will quickly converge to the equilibrium state as workload changes. We found \sys provides high robustness
to bursty short-flow workload, exhibiting a near-optimal flow completion time. We also found \sys provides high per-flow throughput, high bottleneck link 
utilization and small queue at switches, although \sys is not designed to optimize these traditional congestion control metrics.
\item We demonstrate in both packet-level and flow-level simulation that \sys can easily scale to data center size with thousands of servers, while retaining 
its performance gains at the same time. We also demonstrate that \sys is more resilient to packet loss than TCP and is highly resilient to inaccurate flow information.
\item We develop and evaluate a multipath version of \sys. By exploiting path diversity, we demonstrate that multipath \sys further improves its  
performance and reliability from the single-path \sys.
\end{itemize}


\textbf{Outline:} Next, we discuss an example of benefits~(\S\ref{sec:benefits}), followed by a description of design goals~(\S\ref{sec:challenges}).
%challenges to apply scheduling disciplines to data center flows 
We then present \sys protocol~(\S\ref{sec:algorithm}) and its 
basic properties~(\S\ref{sec:properties}). We demonstrate how \sys works~(\S\ref{sec:dynamic}), followed by a thorough 
performance evaluation (\S\ref{sec:evaluation}), and an analysis of failure resilience (\S\ref{sec:badcases}) using both 
packet-level and flow-level simulation. We then extend to Multipath \sys and demonstrate its effectiveness (\S\ref{sec:multipath}).
Finally, we discuss the protocol limitations~(\S\ref{sec:discussion}), related work (\S\ref{sec:relatedwork}) and conclude~(\S\ref{sec:conclusion}).
%present \sys implementation~(\S\ref{sec:implementation}), 
%Finally, we discuss 





==> mattintro.tex <==
\section{Introduction (Matt)}

Datacenters are now used as the underlying infrastructure of many modern
commercial operations, including web services, cloud computing,  and some of
the world's largest databases and storage services.  Because of this, modern
datacenter networks face some of the most large-scale workloads of any network
in existence.  Unfortunately, datacenters also often host applications with
very demanding real-time requirements, including financial services,
multimedia, communications services, and web search.  Meeting these
requirements in this taxing environment is a very challenging problem.

To meet this challenge, we need some way to effectively divide up the bandwidth
of the network across the different jobs that the data center network is
running. To cope with modern datacenters' large-scale workloads, we would like
to maximize the {\em throughput}, or number of jobs that can be completed per
unit time. To cope with datacenters' application demands, we would like to
ensure that the number of jobs that meet application deadlines is as high as
possible.

How can we solve this problem? One approach would be to apply existing
transport mechanisms, such as TCP, RCP, ICTCP, and DCTCP. However, these
mechanisms were designed with a different goal in mind. These approaches work
by targeting {\em fair sharing} of network capacity---link bandwidth is equally
divided across flows.  While fair sharing is a useful approach for environments
where a resource should be divided evenly over participants, for example
environments with uncooperative hosts, fair sharing is known to be far from
optimal in terms of minimizing flow completion time, and the number of flows
that meet their deadlines.

This paper takes a different approach. In particular, we propose \sys, a scheme
that  leverages ideas developed in the context of real-time operating systems
to perform {\em dynamic scheduling} of flows in a data center.  The main
observation is that the problem of optimally scheduling a set of tasks for a
shared resource, with the goal of maximizing throughput, is not a new problem.
In the context of real-time operating systems, a class of {\em dynamic
scheduling algorithms} have been developed that are known to be optimal for
this problem.  For example, the Earliest Deadline First (EDF) dynamic 
scheduling policy, which stores a queue of tasks sorted by deadlines and
repeatedly selects the task with nearest deadline for scheduling, is known to
be optimal: if there is a set of jobs with deadlines, and there exists a
schedule that enables all jobs to be completed before their deadlines, EDF will
complete those jobs by their deadlines.  For tasks without deadlines, Shortest
Job First (SJF) is known to maximize process throughput, as well as minimizing
the amount of time each process needs to wait before its execution is complete.
In addition to providing strong properties, these algorithms are known to significantly
outperform more simple scheduling disciplines, which is reflected by our results,
which show large performance improvements over (non-dynamic) schemes based on FCFS (e.g., D3~\cite{xx}) and fair sharing.

However, dynamic scheduling policies such as EDF and SJF were developed in the
context of centralized environments. Applying these ideas to a distributed
datacenter environment introduces several new challenges.  First, centralized
dynamic scheduling relies on the ability to {\em preempt} an existing task, to
ensure a newly arriving task with a smaller deadline is able to be completed
before a currently-scheduled task. To support this task in distributed
environments, \sys provides the ability to perform distributed preemption of
existing flow traffic, in a manner that enables fast switchover and is
guaranteed not to lead to deadlock.  Second, centralized dynamic scheduling
assumes that the global state of the system is known to the scheduler, and that
scheduling is done at a single point.  To perform dynamic scheduling in
decentralized environments, \sys provides a distributed algorithm to allow a
set of switches to collaboratively gather information about flow workloads, and
converge to a stable agreement on allocation decisions.

Through an extensive simulation study leveraging real datacenter workloads\mattc{are you going to use those Wisc traces?}, we
find that \sys provides strong benefits over existing datacenter transport
mechanisms.  For deadline-constrained flows, \sys outperforms \bntl by
supporting $3$ times more concurrent senders while satisfying their flow
deadlines.  When flows have no deadlines, we show \sys can reduce flow
completion times by $\sim$$30\%$ as compared with TCP and RCP \mattc{and D3?
Can I say D3 here?}. \mattc{any other impressive results you could include here?}

\mattc{I think the name "SCP" is already used for the Secure Copy Protocol. How about we call your scheme WTA for Winner Take All? or how about WTF for Winner Take the Full amount?}

\textbf{Roadmap:} We start by giving a motivating example to demonstrate the
benefits of \sys~(\S\ref{sec:benefits}), followed by a description of our design's
goals~(\S\ref{sec:challenges}).  We then present the details of the \sys
protocol~(\S\ref{sec:algorithm}) and its basic
properties~(\S\ref{sec:properties}). We then give an experimental demonstration to show how \sys
works in practice~(\S\ref{sec:dynamic}), followed by a more detailed performance evaluation
(\S\ref{sec:evaluation}), and an analysis of failure resilience
(\S\ref{sec:badcases}) using both packet-level and flow-level simulation. We
then extend \sys to support multipath forwarding and evaluate its performance
(\S\ref{sec:multipath}).  Finally, we discuss the
limitations of our protocol~(\S\ref{sec:discussion}) and some related work (\S\ref{sec:relatedwork}), and then conclude~(\S\ref{sec:conclusion}).

%       %      \section{Introduction2}
%       %      \label{sec:introduction}
%       %      
%       %      Almost any network flow in data centers is preferable to finish early, as users always want to get their results in the shortest time. 
%       %      Some flows even have specified deadline to meet because of the soft real-time nature of data center applications such as web search, 
%       %      retail, advertising, and recommendation systems. 
%       %      Consequently, a deadline-constrained flow is useful if and only if it completes before the deadline~\cite{dctcp}.
%       %      Unfortunately, transport protocols like TCP are neither minimizing
%       %      flow completion time nor optimizing for deadlines, resulting in the fact that a significant fraction of 
%       %      flow deadlines are missed in today's data centers~\cite{bntl}.
%       %      
%       %      Until now, \emph{fair sharing} -- link bandwidth is equally divided among flows -- 
%       %      is a long-established objective adopted by current congestion control protocols in data centers 
%       %      such as TCP, RCP\cite{rcp}, ICTCP~\cite{ictcp} and DCTCP~\cite{dctcp}. 
%       %      In particular, these protocols will gradually converge on the fair-share allocation among flows.
%       %      However, fair sharing is known to be far from optimal in terms of minimizing flow completion time~\cite{PShaslargeFCT} 
%       %      and the number of deadline-missing flows~\cite{EDFbetterthanPS}.
%       %      %\cut{XCP\cite{xcp}}
%       %      
%       %      Arguably, \emph{flow scheduling}\footnote{We refer flow scheduling to sequencing flow transmission order in \emph{time}. 
%       %      This differs from the flow scheduler in Hedera~\cite{hedera} which assigns flows to \emph{paths}.} 
%       %      is the most persuasive solution to this problem:
%       %      Rather than allowing all flows to transmit at the same time, one 
%       %      could leverage scheduling theory to resequence flow transmission order, 
%       %      achieving optimum in many scenarios. 
%       %      Consider a single bottleneck link: Transmitting flows one after one in increasing order of flow 
%       %      size (Shortest Job First; SJF) is optimal to minimize average flow completion time~\cite{srptoptimality};
%       %      if flows are annotated with deadlines, transmitting flows in increasing order 
%       %      of deadline (Earliest Deadline First; EDF) is optimal to find a deadline-satisfying solution if any exists~\cite{edfoptimality}.
%       %      As we will show in later section, these scheduling disciplines have clear performance advantages over 
%       %      existing congestion control protocols even for more complex scenarios (e.g., multi-rooted tree topology, dynamic traffic loads).
%       %      
%       %      %In this paper we start with the assumptions that \textbf{\small(i)} minimizing flow completion time (for flows without deadline) and 
%       %      %satisfying flow deadline requirements (for deadline-constrained flows) at the same time 
%       %      %plays an important, perhaps even necessary, role in data center networks, and \textbf{\small(ii)} the use of fair sharing in existing transport protocols is 
%       %      %a substantial hindrance to achieve this goal.
%       %      %We are not claiming that they are true, but rather are only 
%       %      %looking at the implications if indeed they are true by using these two
%       %      %assumptions as our starting points. If one starts with these assumptions, 
%       %      %then designing a new congestion control protocol to achieve this goal becomes a very important issue.
%       %      
%       %      %To address this problem, 
%       %      %this paper develops a novel protocol for congestion control that
%       %      %outperforms state-of-the-art transport protocols in data center networks.
%       %      
%       %      Since it seems that \emph{fair} sharing hinders flow completion time, we propose the opposite: 
%       %      giving high priority to certain flows chosen by a scheduling discipline. 
%       %      This Scheduling-based transmission Control Protocol (\textbf{\sys{}}) is 
%       %      %, outperforms state-of-the-art congestion control protocols in data center networks, 
%       %      efficient, error-resilient, and scalable to current data center size. 
%       %      It borrows the ideas from centralized scheduling disciplines and 
%       %      implements it in a fully distributed manner. 
%       %      With explicit rate control, \sys can approximate a range of scheduling disciplines by 
%       %      suitably manipulating the flow transmission time. To achieve this, 
%       %      \sys exhibits a unique feature that differentiates it from other congestion control protocols.
%       %      We refer this feature as \emph{preemption}:
%       %      A scheduling discipline first defines how critical a network flow is, and \sys is capable to give 
%       %      priority to the most critical flows while pausing the other contending flows at 
%       %      the same time regardless of flow arrival time. This distinctive feature substantially influences the performance: 
%       %      In a deadline-constrained case, an urgent flow can ``preempt'' other flows to meet its deadline constraint. 
%       %      As we will later show, preemption is very useful to minimize flow completion time even when flows have no deadlines.
%       %      
%       %      To schedule flow transmission time, \sys switches collaboratively converge to a stable agreement and 
%       %      inform the senders about the time to start their transmission.
%       %      By putting flow information in the packets,
%       %      switches need no additional standalone control message, maintain no per-flow state, use only FIFO tail-drop queue and require no synchronized clock.
%       %      
%       %      Like D$^3$, a recent deadline-agnostic protocol proposed by Wilson et al.~\cite{bntl}, 
%       %      \sys requires flow information like flow size and deadline at flow initiation time. 
%       %      Unlike D$^3$, which is in spirit a first-come first-serve algorithm, \sys gives network resources to the most critical 
%       %      flow, approximating the optimal schedule and outperforming D$^3$.
%       %      We discuss in~\S\ref{sec:discussion} why the flow size information is available in data center networks, and 
%       %      even if this information is inaccurate, we show that \sys performance will 
%       %      degrade slowly and gracefully as inaccuracy increases in~\S\ref{sec:badcases}.
%       %      
%       %      Through both packet-level and flow-level simulation, we observe clear benefits at many network sizes, ranging from a single 
%       %      bottleneck topology to a Fat-tree~\cite{fattree} topology with thousands of servers. 
%       %      Inspired by recent proposal on multipath TCP~\cite{mptcp,mptcp-nsdi}, we also develop a multipath version of \sys in \S\ref{sec:multipath}.
%       %      By exploiting path diversity, the multipath \sys further improves reliability and flow completion time from the single-path \sys.
%       %      
%       %      %We looked at BCube~\cite{bcube}, multi-homed data center topologies, to take advantage of parallel paths between hosts.
%       %      %In random permutation traffic, we show that $4$-subflow \sys can support twice the number of concurrent flows with tight deadlines than single-path \sys.
%       %      
%       %      In summary, our key contributions include:
%       %      \begin{itemize}
%       %      \item We design and implement \sys, a fully distributed protocol that optimizing flow completion time in data centers based on scheduling disciplines.
%       %      \item We have examined many traffic patterns and topologies, and in 
%       %      all of them \sys provides significant advantages over state-of-the-art congestion control protocols.
%       %      For deadline-constrained flows, \sys outperforms \bntl in supporting $3$ times
%       %      more concurrent senders while satisfying their flow deadlines. 
%       %      When flows have no deadlines, we show \sys can save $\sim$$30\%$ average flow
%       %      completion time compared with TCP and RCP.
%       %      \item We show that \sys has no deadlock and will quickly converge to the equilibrium state as workload changes. We found \sys provides high robustness
%       %      to bursty short-flow workload, exhibiting a near-optimal flow completion time. We also found \sys provides high per-flow throughput, high bottleneck link 
%       %      utilization and small queue at switches, although \sys is not designed to optimize these traditional congestion control metrics.
%       %      \item We demonstrate in both packet-level and flow-level simulation that \sys can easily scale to data center size with thousands of servers, while retaining 
%       %      its performance gains at the same time. We also demonstrate that \sys is more resilient to packet loss than TCP and is highly resilient to inaccurate flow information.
%       %      \item We develop and evaluate a multipath version of \sys. By exploiting path diversity, we demonstrate that multipath \sys further improves its  
%       %      performance and reliability from the single-path \sys.
%       %      \end{itemize}
%       %      
%       %      
%       %      \textbf{Outline:} Next, we discuss an example of benefits~(\S\ref{sec:benefits}), followed by a description of design goals~(\S\ref{sec:challenges}).
%       %      %challenges to apply scheduling disciplines to data center flows 
%       %      We then present \sys protocol~(\S\ref{sec:algorithm}) and its 
%       %      basic properties~(\S\ref{sec:properties}). We demonstrate how \sys works~(\S\ref{sec:dynamic}), followed by a thorough 
%       %      performance evaluation (\S\ref{sec:evaluation}), and an analysis of failure resilience (\S\ref{sec:badcases}) using both 
%       %      packet-level and flow-level simulation. We then extend to Multipath \sys and demonstrate its effectiveness (\S\ref{sec:multipath}).
%       %      Finally, we discuss the protocol limitations~(\S\ref{sec:discussion}), related work (\S\ref{sec:relatedwork}) and conclude~(\S\ref{sec:conclusion}).
%       %      %present \sys implementation~(\S\ref{sec:implementation}), 
%       %      %Finally, we discuss 
%       %      
%       %      



==> properties_old.tex <==
\section{\sys Properties}
\label{sec:properties}

We first present two important properties of \sys.

\newtheorem{theorem}{Property}
\begin{theorem}
\textnormal{
\sys has no deadlock.
}
\end{theorem}
\begin{proof}
Deadlock in transport protocol is a situation where two or more competing flows are each waiting for the other to 
finish, and therefore neither ever does. We ensure \sys has no deadlock by showing that a necessary condition of 
deadlock, Hold and Wait, is false. If a \sys flow is paused, the switch who pauses this 
flow will update the blockby field in the scheduling header (\pausebyh) to its ID.
This blocking information will eventually reach all the other switches along the path. Even if packet loss happens, 
the same switch will update the blockby field on the next packet sent by the sender of the paused flow.
Whenever a switch notices that a flow is paused by another switch, it will not accept this flow and simply bypass the request.
Thus, a paused flow will not hold the resource from \emph{any} switch.
\end{proof}

\begin{theorem}
\textnormal{
When network workload changes, \sys will converge to equilibrium. The convergence time is less than $3$ RTTs when there is no packet loss.
}
\end{theorem}
\begin{proof}
We say a flow is a \emph{driver} if it is more critical than any other flow that shares at least one common link with it. 
Given a set of active flows, we define the equilibrium as a state where the drivers are sending data while the remaining flows are paused.
When a driver arrives, we usually need one RTT latency before the sender can start sending. 
In the worst case it could take up to two RTTs because of flow dampening: a RTT for switches to store the flow, and an additional 
RTT for switches to accept the driver. After switches accept the driver, we need at most one RTT for the other non-driver flows 
to stop sending after receiving the updated feedback.
Thus, \sys will converge in at most $3$ RTTs when there is no packet loss. 
When packet loss exists, we need additional latency for senders to send next packets. 
As long as packet dropping rate is not $100$\%, \sys will converge to equilibrium in finite time.
\end{proof}

We now demonstrate how \sys works through packet-level simulation using two simple scenarios, and 
we will present detailed evaluation in the following sections. 
The experiments are conducted by assuming a single bottleneck topology with a NIC rate of $1$Gbps \cut{(Figure~\ref{topology:simple})}.
We measured flow throughput (the per-flow number of successfully ACK'ed bits, excluding protocol overhead), 
link utilization (the number of delivered bits), and the instantaneous queue (the number of data packets). 
 
\textbf{Scenario 1 (Convergence Dynamics):} Figure~\ref{fig:case1} shows that \sys provides seamless flow switching. 
We assume five flows that start at time $0$. The flows have no deadline, and each flow has a size of $\sim$$1$ MByte.
The flow size is perturbed slightly such that a flow with smaller index is more critical. 
Ideally, the five flows together take $40$ ms to finish because each flow requires a raw processing time of $\frac{1\textrm{~MB}}{1\textrm{~Gbps}} = 8\textrm{~ms}$. 
With seamless flow switching, \sys completes at $\sim$$42$ ms due to protocol 
overhead ($\sim$$3\%$ bandwidth loss due to TCP/IP header) and first-flow initialization time (two-RTT latency loss; one RTT latency for the sender to receive the SYN-ACK, 
and an additional RTT for the sender to receive the first DATA-ACK). 
We observe that \sys can converge to equilibrium quickly at flow switching time, 
resulting in a near perfect ($100\%$) bottleneck link utilization (Figure~\ref{fig:b_util}).
Although one naive approach to achieve such high link utilization is to let 
multiple flows send data concurrently, it causes the rapid growth of the queue and 
potentially leads to congestive packet loss.
Unlike this approach, \sys exhibits very small queue size 
and has no packet drops (Figure~\ref{fig:b_queue}). 
The non-integer values in the y axis comes from the small-size control packets like probes.

\begin{figure}[t]
\centering
\subfloat[]{ \label{fig:b_throughput}   \includegraphics[width=3.2in]{fig/b_throughput.pdf}}\vspace{-13pt}\\
\subfloat[]{ \label{fig:b_util}   \includegraphics[width=3.2in]{fig/b_util.pdf}}\vspace{-13pt}\\
\subfloat[]{ \label{fig:b_queue}   \includegraphics[width=3.2in]{fig/b_queue.pdf}}\vspace{-12pt}
\caption{\figtitle{\sys provides seamless flow switching. It achieves high link utilization at flow switching time, maintains small queue, and converges 
to the equilibrium quickly.}}
\label{fig:case1}
\end{figure}

\textbf{Scenario 2 (Robustness to Burst):} Figure~\ref{fig:case2} shows that \sys provides high robustness to bursty workload. 
We assume a background long flow that starts at time $0$, and $50$ short flows that all start at $10$ ms. 
The short flow sizes are set to $20$KByte with small random perturbation.
Figure~\ref{fig:m_throughput} shows that \sys adapts quickly to sudden burst of short flows.
Because the required delivery time of each short flow is very small ($\frac{20\textrm{~KByte}}{1\textrm{~Gbps}} \approx 153$ $\mu$s), 
the system never reaches stable state during the preemption period (between $10$ and $19$ ms).
Figure~\ref{fig:m_util} shows that \sys exhibits high utilization with very limited oscillations:
the average link utilization during the preemption period is $91.7\%$.
Moreover, Figure~\ref{fig:m_util} demonstrates that \sys lets short flows send one after one, resulting in near-optimal average completion time.
Figure~\ref{fig:m_queue} suggests that \sys does not compromise the queue length. By contrast, XCP results in a queue of $\sim$$60$ packets when encountering 
a burst of flows (Figure 11(b) in~\cite{xcp}). 

\begin{figure}[t]
\centering
\subfloat[]{ \label{fig:m_throughput}   \includegraphics[width=3.2in]{fig/m_throughput.pdf}}\vspace{-13pt}\\
\subfloat[]{ \label{fig:m_util}   \includegraphics[width=3.2in]{fig/m_util.pdf}}\vspace{-13pt}\\
\subfloat[]{ \label{fig:m_queue}   \includegraphics[width=3.2in]{fig/m_queue.pdf}}\vspace{-12pt}
\caption{\figtitle{\sys exhibits high robustness to bursty workload. 
We assume $50$ concurrent short flows, all initiating at time $1$ ms to preempt a background long flow.}}
\label{fig:case2}
\end{figure}


